A Data Annotation Requirements Representation and Specification (DARS)

With the rise of AI-enabled cyber-physical systems, data annotation has become a critical yet often overlooked process in the development of these intelligent information systems. Existing work in requirements engineering (RE) has explored how requirements for AI systems and their data can be represented. However, related interviews with industry professionals show that data annotations and their related requirements introduce distinct challenges, indicating a need for annotation-specific requirement representations. We propose the Data Annotation Requirements Representation and Specification (DARS), including an Annotation Negotiation Card to align stakeholders on objectives and constraints, and a Scenario-Based Annotation Specification to express atomic and verifiable data annotation requirements. We evaluate DARS with an automotive perception case related to an ongoing project, and a mapping against 18 real-world data annotation error types. The results suggest that DARS mitigates root causes of completeness, accuracy, and consistency annotation errors. By integrating DARS into RE, this work improves the reliability of safety-critical systems using data annotations and demonstrates how engineering frameworks must evolve for data-dependent components of today's intelligent information systems.

==> CutParts/AccuracyTable.tex <==
{
\begin{table}[]
%\vspace{-0.5cm}
    \centering
\scriptsize
\begin{talltblr}[
  caption = {Possible Mitigation of Data Annotation Accuracy Errors (C: Annotation Negotiation Card, S: Scenario-Based Annotation Requirement Specification)},
  label = {tab:accuracyMap}
]{
  width = \linewidth,
  colspec = {X[1,l,t] X[1.2,l,t] X[3,l,t]},
  cell{2}{1} = {r=3}{},
  cell{5}{1} = {r=3}{},
  cell{5}{3} = {r=2}{},
  cell{8}{1} = {r=2}{},
  cell{8}{3} = {r=2}{},
  cell{10}{1} = {r=3}{},
  cell{13}{1} = {r=3}{},
  vline{2-3} = {-}{solid},
  hline{1-2,5,8,10,13,16} = {-}{},
  hline{3-4,7,11-12,14-15} = {2-3}{},
  hline{6,9} = {2}{},
}
\textbf{Accuracy errors} & \textbf{Causes} & \textbf{Mitigation}\\
Wrong class label & Ambiguous class boundaries & S: Explicitly define boundaries with the aid of exception and edge-case scenario requirements.\\
 & Fatigue & N/A\\
 & Limited quality assurance & C: Quality Assurance \& Feedback Protocol, mandate regular check-ins to catch systematic class errors.\\
Bounding-box errors & Weak quality assurance tolerances & S: the optional \textless{}constraint\textgreater{} can be used to define measurable precision (e.g., ``2px margin''). The Acceptance criteria helps define metrics over bounding box quality.\\
 & Subjective edges & \\
 & Tool instability & N/A\\
Granularity mismatch & Outdated/misaligned taxonomy & {C: Tooling, Taxonomy \& Hand-off, defines a shared Taxonomy/Ontology, the detailed levels can be negotiated here as well.\\S: The standard scenario type annotation requirement can also be used to demonstrate the depth of annotation detail.}\\
 & Inconsistent detail levels & \\
Insufficient guidance & Vague/incomplete docs & C \& S are both docs with atomic, testable scenarios providing guidance to annotators.\\
 & No versioning & C: Guideline Governance defines versioning.\\
 & Limited feedback & C: Quality Assurance \& Feedback Protocol, establish feedback loop to clarify annotation requirements.\\
Bias-driven errors & Unbalanced data & C: Operational context \& Representation plan, enforces a specific quota and diversity target before data is collected or annotated.\\
 & Automation over-trust & N/A\\
 & Cognitive bias & N/A
\end{talltblr}
%\vspace{-.5cm}
\end{table}
}

==> CutParts/ConsistencyTable.tex <==

{
\begin{table}[]
\centering
\scriptsize
\begin{talltblr}[
  caption = {Possible Mitigation of Data Annotation Consistency Errors (C: Annotation Negotiation Card, S: Scenario-Based Annotation Requirement Specification)},
  label = {tab:consistencyMap}
]{
  width = \linewidth,
  colspec ={X[1,l,t] X[1.2,l,t] X[3,l,t]},
  cell{2}{1} = {r=3}{},
  cell{2}{3} = {r=2}{},
  cell{5}{1} = {r=2}{},
  cell{7}{1} = {r=2}{},
  cell{9}{1} = {r=2}{},
  cell{9}{3} = {r=2}{},
  cell{11}{1} = {r=2}{},
  cell{13}{1} = {r=2}{},
  cell{13}{3} = {r=2}{},
  cell{15}{1} = {r=2}{},
  cell{15}{3} = {r=2}{},
  vline{2-3} = {-}{solid},
  hline{1-2,5,7,8,9,10,11,13,15,17} = {-}{},
  hline{3,14,16} = {2}{},
  hline{4,6,12} = {2-3}{},
}
\textbf{Consist. errors} & \textbf{Causes} & \textbf{Mitigation}\\
Inter-annotator disagreement & Subjective judgments & S: Removes subjectivity by defining measurable limits (e.g., ``occlusion $>$ 50\%'')or precise annotation constraints (e.g., ``Box must include estimated feet'').\\
 & Ambiguous rules & \\
 & Limited quality assurance cycles & C: Quality assurance \& Feedback protocol, regular agreed upon review cycles that are within negotiated cost-driven limits.\\
Ambiguous instructions & Unclear/ contradictory/ overlong guidelines & In addition to the overall guidance of C, atomic requirements with vertical traceability could avoid contradictions.\\
 & Missing context & S: templates contains specific context field, with visual example.\\
Lack of purpose knowledge & Poor comms of downstream goals & C: System \& model objectives, S: Vertical traceability is provided to link each requirement back to negotiated agreements in C, Rationale is also communicated.\\
 & Limited onboarding & Both C \& S can both serve as structured onboarding documents.\\
Misaligned hand-offs & Under-documented transitions & C: Tooling, taxonomy \& hand-off, defines hand-off protocol and specifies transfer formats.\\
 & Multi-vendor rule drift & \\
Limited review  logging & Scarce quality assurance automation & N/A\\
 & No traceability/versioned checks & C: Quality assurance \& feedback, provides defined review cadence. S: Acceptance criteria makes every requirement verifiable.\\
Lack of framework/ standards & No shared ontology/benchmarks & C: Tooling, taxonomy \& hand-off, mandates the definition of a agreed upon project-specific Taxonomy/ontology to replace currently missing industry standards and benchmarks.\\
 & Uneven standard adoption & \\
Cross-modality misalignment & Calibration/sync gaps & C: Tooling, taxonomy \& hand-off, define sensor synchronization and calibration rules before annotation begins.\\
 & Weak 3D to 2D projection validation & 
\end{talltblr}

\end{table}
}

==> CutParts/Limitations.tex <==
\subsubsection{Limitations}
While our two artifacts provide possibilities to mitigate many annotation errors, we acknowledge several limitations rooted in human factors and infrastructure constraints that documentation artifacts cannot directly resolve.

First, errors caused by human factors such as ``annotator fatigue'', ``automation over-trust'' and ``cognitive bias'' (\textit{Wrong class labels}, \textit{Bias-driven errors}, \textit{Attribute omission}) are difficult to eliminate through requirements alone. While our atomic, scenario-based structure could reduce the cognitive load that contributes to these errors, it cannot physically prevent fatigue or subconscious bias.

Second, errors caused by infrastructure gaps such as ``tool instability'' (\textit{Bounding-box errors}) or ``scarce quality assurance automation'' (\textit{Limited review logging}) are technical constraints. Our artifacts cannot invent automation where non currently exist. Our solution however, might mitigate the impact of these limitations: the \textbf{Tooling} negotiation field of the Card allows team to disqualify unstable tools during the selection process, and \textbf{Quality assurance \& feedback protocol} ensures that whatever limited review resources are available are allocated systematically.

Finally, while the Card can mandate compliance features (e.g., audit logs) to prevent \textit{Privacy omissions}, the enforcement of these features relies on the tool provider's capabilities.


==> CutParts/SpaceFigure.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{multilayerconcept.png}
    \vspace{-1em}\caption{Problem space and data space conceptualization from~\cite{dey2023multi}. \vspace{-1em}}
    \label{fig:multilayerconcept}
\end{figure*}
The framework consists of three layers: a \emph{Problem layer} (problem space), a \emph{Data layer} (data space) and an \emph{Evidence layer} (evidence combination and uncertainty assessment). 

==> CutParts/methodology.tex <==
\section{Methodology}\label{sec:methodology}
The overarching research work follows a design science research (DSR) approach with iterative cycles of problem exploration, artifact design, and preliminary evaluation~\cite{wieringa2014design}.
In this paper, we present the result of the first cycle of this work outlined in Figure~\ref{fig:methodflow}.
\begin{figure*}[b]
    \centering
    \includegraphics[width=\linewidth]{Method_Flow.pdf}
    \vspace{-2em}
    \caption{Overview of methodological steps and their key outputs.}
    \label{fig:methodflow}
    \vspace{-1.5em}
\end{figure*}
First, we conducted a \emph{problem exploration} based on ongoing work with industry on data annotation and RE in automotive perception~\cite{hinaICSEJSS,saeeda2025requirements}.
We compared findings in this ongoing project with existing RE-for-ML and data-requirements approaches outlined in Section~\ref{sec:background} to identify a gap relating to explicating data annotation requirements. Then, in a second step, we performed a \emph{grounded requirement analysis} to suggest solutions.
Together with industry experts, we derived design criteria for a representation that must support traceability to system goals, verifiability through evidence, explicit treatment of edge cases and exception, and alignment between strategic agreements and operational annotation practice. 
The experts from an automotive OEM, Tier-1 supplier, as well as a data annotation company were recruited from the ongoing research project FAMER\footnote{\url{https://ffi-famer.github.io/}}. In a third step, we conducted a \emph{concept synthesis and artifact design} together with the company experts.
We combined ideas from MLTE Negotation Cards~\cite{mlte_negotiation_card}, the multi-layered data requirements framework~\cite{saeeda2025requirements}, and pattern-based requirement templates~\cite{peng2025mlreqs}. 
Through discussions with the company experts and repeated alignment against known challenges within the companies, we iteratively arrived at two complementary artifacts: the Annotation Negotiation Card and the Scenario-based Annotation Specification. We then, in a fourth step, performed \emph{scenario construction and specification} in which we defined three scenario types: common (standard), ambiguous (edge-cases), and exclusion (exceptions) situations in annotations. 
For each type, we instantiated the Scenario-based Annotation Specification to obtain atomic and testable annotation requirements.
For an initial \emph{validation through demonstration} we applied in a fifth step the resulting artifacts from steps three and four to a realistic Automatic Emergency Braking (AEB) perception system scenario inspired by a current existing safety case~\cite{borg2023ergo}.
Then, in a final step to further strengthen the validation, we conducted an \emph{analytical evaluation} against the taxonomy of 18 data annotation errors~\cite{hinaCAIN}.
We systematically mapped each error and its reported root cause to concrete elements of our two suggested artifacts. 
We used this mapping then to reason about which errors could be mitigated by EARR and which remain depending on human and tooling factors. 
The outcome of this mapping also informed the discussion of limitations and guide directions for further empirical and industrial validation. 






